G3PO: Leveraging a Hybrid Use of Verifiability and Preference in Reinforcement Learning

Reinforcement Learning with Verifiable Rewards (RLVR) has shown strong performance in eliciting reasoning in LLMs on tasks with deterministic outcomes, while Reinforcement Learning from Human Feedback (RLHF) has remained a viable option for more subjective, reasoning-based tasks. This is especially true when paired with Process Reward Models (PRMs), which are generally trained on human preference data and are increasingly used to shape policy optimisation. However, the two signals are rarely combined beyond a weighted sum, and little work has investigated whether doing so would lead to more stable training signals. To address this gap, we introduce Group verifiability-Prioritised Preference Policy Optimisation (G3PO), a lexicographic policy optimisation strategy that ranks completions first by verifiable correctness and then by PRM preference. We evaluate G3PO on three tasks: Medical Risk of Bias Assessment, Medical Reasoning, and Mathematics. Across these domains, our hybrid strategy is shown to consistently improve on standard baselines as well as domain-specific alternatives, demonstrating that prioritising correctness while preserving preference order yields stronger and more effective training signals.

==> diagrams/advantage_bound.tex <==
% Worst-case |A| in a group vs group size G (analytic).
% GRPO, binary correctness reward, z-score with population std: a lone correct
% (or incorrect) completion gets |A| = sqrt(G-1).
% G3PO: rank-based, |A| <= 2 for every G.
\begin{tikzpicture}
\definecolor{colorG3PO}{HTML}{8A2BE2}
\definecolor{colorGRPO}{HTML}{FF8C00}
\begin{axis}[
    width=0.97\columnwidth,
    height=0.58\columnwidth,
    xlabel={Group size $G$},
    ylabel={Worst-case $\max_i |A_i|$},
    xmode=log, log basis x=2,
    xmin=2, xmax=32,
    ymin=0, ymax=6,
    xtick={2,4,8,16,32},
    xticklabels={2,4,8,16,32},
    ytick={0,1,2,3,4,5,6},
    tick label style={font=\scriptsize},
    label style={font=\footnotesize},
    axis line style={black!60},
    tick style={black!60},
    major tick length=2pt,
    grid=major,
    grid style={black!12, line width=0.3pt},
    every axis plot/.append style={line width=1.0pt, line join=round},
    clip=false,
]
\addplot[draw=none, fill=colorG3PO, fill opacity=0.10, domain=2:32, samples=2] {2} \closedcycle;
\addplot[colorG3PO, line width=1.2pt, domain=2:32, samples=2] {2};

\addplot[colorGRPO, domain=2:32, samples=80, smooth] {sqrt(x-1)};
\addplot[colorGRPO, only marks, mark=*, mark size=1.4pt, samples at={2,4,8,16,32}] {sqrt(x-1)};

\draw[black!45, dash pattern=on 1.5pt off 1.5pt, line width=0.5pt]
    (axis cs:8,0) -- (axis cs:8,6);
\node[font=\tiny, text=black!60, anchor=south west, inner sep=1pt, fill=white, fill opacity=0.85, text opacity=1]
    at (axis cs:8,5.25) {$G=8$ (ours)};

\node[font=\scriptsize, text=colorGRPO!85!black, anchor=north west, inner sep=1.5pt]
    at (axis cs:10.5,3.05) {GRPO: $\sqrt{G-1}$};
\node[font=\scriptsize, text=colorG3PO!85!black, anchor=north east, inner sep=1.5pt]
    at (axis cs:31,1.95) {G3PO: $\le 2$};
\node[font=\tiny, text=colorGRPO!85!black, anchor=south east, inner sep=1pt]
    at (axis cs:8,2.70) {$\sqrt7$};
\end{axis}
\end{tikzpicture}

